Long-context LLMs Struggle with Long In-context Learning

Large Language Models (LLMs) have made significant strides in handling long sequences. Some models like Gemini could even to be capable of dealing with millions of tokens. However, their performance evaluation has largely been confined to metrics like perplexity and synthetic tasks, which may not fully capture their true abilities in more challenging, real-world scenarios. We introduce a benchmark (LongICLBench) for long in-context learning in extreme-label classification using six datasets with 28 to 174 classes and input lengths from 2K to 50K tokens. Our benchmark requires LLMs to comprehend the entire input to recognize the massive label spaces to make correct predictions. We evaluate on 15 long-context LLMs and find that they perform well on less challenging classification tasks with smaller label space and shorter demonstrations. However, they struggle with more challenging task like Discovery with 174 labels, suggesting a gap in their ability to process long, context-rich sequences. Further analysis reveals a bias towards labels presented later in the sequence and a need for improved reasoning over multiple pieces of information. Our study reveals that long context understanding and reasoning is still a challenging task for the existing LLMs. We believe LongICLBench could serve as a more realistic evaluation for the future long-context LLMs.

==> Sections/NERD_results.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{5K}} &\multicolumn{1}{c}{\textbf{9K}}  &\multicolumn{1}{c}{\textbf{14K}}    &\multicolumn{1}{c}{\textbf{19K}}  &\multicolumn{1}{c}{\textbf{24K}} \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8k & \textbf{44.0}  & 44.2	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32k & 36.9  & 40.8	& 41.1	& 41.6	& 41.3	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32k & 24.1  & 9.3	& 23.6	& 10.4	& 1.1  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32k & 40.0  & 46.4	& 47.6	& 47.3	& 47.8 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 42.2 & \textbf{47.4}  & \textbf{48.9}	& \textbf{50.0}	& \textbf{50.0} \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200k & 34.3  & 40.2	& 44.8	& 42.3	& 43.2 \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200k & 43.6  & 46.2	& 46.5	& 47.8	& 48.3 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 22.3  & 25.5	& 26.5	& 29.4	& 27.0  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 1k & 13.9  & 0	& 0	& 0.7	& 9.9 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2k & 0  & 0	& 0	& 0	& 0 \\
\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32k & 36.8  & 26.1	&  28.5	&  27.4	&  28.4 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128k & \textbf{53.4}  & \textbf{55.3}	&  \textbf{56.2}	&  \textbf{55.6}	& \textbf{56.8} \\

\midrule
\multicolumn{1}{l}{SoTA (PL-Marker)} & N/A & - & \multicolumn{5}{c}{\textbf{70.9}} \\

\bottomrule
\end{tabular}
\caption{Few-NERD Result.}
\label{table:fewnerd_result}
\end{table}

==> Sections/go_emotion_results.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{0.8K}} &\multicolumn{1}{c}{\textbf{1.6K}}  &\multicolumn{1}{c}{\textbf{2.4K}}    &\multicolumn{1}{c}{\textbf{3.2K}}  &\multicolumn{1}{c}{\textbf{4K}}  \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 0  & 0	& 0	& 0.2	& 0.2	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & \textbf{22.0}  & 17.0	& 15.0	& 12.6	& 10.6  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 14.8  & \textbf{18.2}	& \textbf{18.6}	& \textbf{19.0}	& \textbf{14.2} \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 2.6  & 11.4	& 7.4	& 11.6	& 12.4 \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 0  & 0	& 0.8	& 4.0	& 4.0 \\

% \multicolumn{1}{l}{Baichuan2-7B-Base} & 7B & 4k & 3.2  & 2.8 & 4.4	& 4.2	& 5.2 \\
\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 0  & 0	& 0	& 0.2	& 0.4  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 8.8  & 7.4	& 4.6	& 5.2	& 4.0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\
\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K &  20.3  & 21.4	& 22.4	& 24.4	& 24.0 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{36.5}  & \textbf{34.4}	&  \textbf{35.0}	&  \textbf{33.3}	& \textbf{32.0} \\

\midrule
\multicolumn{1}{l}{SoTA (BERT)} & N/A & - & \multicolumn{5}{c}{\textbf{58.9}} \\

\bottomrule
\end{tabular}
\caption{GoEmotion Result.}
\label{table:goemo_result_new}
\end{table}

==> Sections_old/NERD_results.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{5K}} &\multicolumn{1}{c}{\textbf{9K}}  &\multicolumn{1}{c}{\textbf{14K}}    &\multicolumn{1}{c}{\textbf{19K}}  &\multicolumn{1}{c}{\textbf{24K}} \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8k & \textbf{44.0}  & 44.2	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32k & 36.9  & 40.8	& 41.1	& 41.6	& 41.3	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32k & 24.1  & 9.3	& 23.6	& 10.4	& 1.1  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32k & 40.0  & 46.4	& 47.6	& 47.3	& 47.8 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 42.2 & \textbf{47.4}  & \textbf{48.9}	& \textbf{50.0}	& \textbf{50.0} \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200k & 34.3  & 40.2	& 44.8	& 42.3	& 43.2 \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200k & 43.6  & 46.2	& 46.5	& 47.8	& 48.3 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 22.3  & 25.5	& 26.5	& 29.4	& 27.0  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 1k & 13.9  & 0	& 0	& 0.7	& 9.9 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2k & 0  & 0	& 0	& 0	& 0 \\
\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32k & 36.8  & 26.1	&  28.5	&  27.4	&  28.4 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128k & \textbf{53.4}  & \textbf{55.3}	&  \textbf{56.2}	&  \textbf{55.6}	& \textbf{56.8} \\

\midrule
\multicolumn{1}{l}{SoTA (PL-Marker)} & N/A & - & \multicolumn{5}{c}{\textbf{70.9}} \\

\bottomrule
\end{tabular}
\caption{Few-NERD Result.}
\label{table:fewnerd_result}
\end{table}

==> Sections_old/banking_results.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{2K}} &\multicolumn{1}{c}{\textbf{4K}}  &\multicolumn{1}{c}{\textbf{7K}}    &\multicolumn{1}{c}{\textbf{9K}}  &\multicolumn{1}{c}{\textbf{14K}}  \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & \textbf{30.2}  & \textbf{70.4} & \textbf{72.0}	& \textbf{75.6}	& \textbf{77.2}	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & 16.6  & 23.2	& 22.4	& 22.8	& 8.8  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 21.6  & 52.8	& 61.4	& 66.0	& 67.8 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 29.8  & 43.6	& 66.4	& 67.8	& 64.0 \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 25.8  & 0	& 0	& 0	& 1.2 \\

% \multicolumn{1}{l}{Baichuan2-7B-Base} & 7B & 4k & 3.2  & 2.8 & 4.4	& 4.2	& 5.2 \\
\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 5.6  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 3.0  & 19.4	& 28.0	& 31.6	& 32.6  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 8.6  & 21.2	& 0.4	& 0	& 0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\


\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 33.4  & 41.4	& 40.6	&  45.6	& 50.2 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{73.5}  & \textbf{80.5}	& \textbf{82.0}	&  \textbf{83.5}	&  \textbf{84.4} \\

\midrule
\multicolumn{1}{l}{SoTA (RoBERTA + ICDA)} & N/A & - & \multicolumn{5}{c}{\textbf{94.4}} \\

\bottomrule
\end{tabular}
\caption{BANKING77 Result.}
\label{table:bank77_result_new}
\end{table}

==> Sections_old/dialogre_results.tex <==

\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{8K}} &\multicolumn{1}{c}{\textbf{13K}}  &\multicolumn{1}{c}{\textbf{19K}}    &\multicolumn{1}{c}{\textbf{25K}}  &\multicolumn{1}{c}{\textbf{32K}}               \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 16.3 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 6.9 & 13.9	& 6.3	& 5.7	& 5.9\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & 5.1 & 8.9	& 8.8	& 12.4	& 10.4  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 14.4 & 18.4	& 15.5	& 16.4	& 13.2 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & \textbf{24.3} & \textbf{23.2}	& \textbf{23.4}	& \textbf{22.3}	& \textbf{21.2} \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 0 & 0	& 0.8	& 0.8	& 0 \\

% \multicolumn{1}{l}{Baichuan2-7B-base} & 7B & 192K & 0 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 12.2 & 13.4 & 6.4 & 2.1 & 1.1 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 4.0 & 3.8	& 3.0	& 6.4	& 2.2 \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 0 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0 & 0	& 0	& 0	& 0 \\

\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 23.6 & 29.2	& 33.2	& 26.1	& 17.3 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{43.5} & \textbf{48.8} & \textbf{53.6} & \textbf{60.2} & \textbf{60.9} \\

\midrule

\multicolumn{1}{l}{SoTA (HiDialog)} & N/A & - & \multicolumn{5}{c}{\textbf{77.1}} \\

\bottomrule
\end{tabular}
\caption{DialogRE Result.}
\label{table:tacred_result}
\end{table}

==> Sections_old/discovery_ablation.tex <==
% \begin{table}[!thb]
%     \small
%     \centering
%     \begin{tabular}{lccccccccc}
%     \toprule
%     \multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Label Instruction}}
%     &\multicolumn{1}{c}{\textbf{2k}} &\multicolumn{1}{c}{\textbf{5k}}  &\multicolumn{1}{c}{\textbf{10k}}    &\multicolumn{1}{c}{\textbf{15k}}  &\multicolumn{1}{c}{\textbf{20k}}   &\multicolumn{1}{c}{\textbf{25k}} &\multicolumn{1}{c}{\textbf{32k}}               \\
%     \midrule
%     \multicolumn{1}{l}{LLaMA-2-7B-32K} & - & 2.4 & 3.2 & 3.0 &	3.8 &	3.8 & 3.8 &	2.8   \\
%     \multicolumn{1}{l}{} & \checkmark & 4.4 & 3.8 & 3.2 &	4.0 &	4.0 & 3.8 &	4.0   \\
%     \midrule
%     \multicolumn{1}{l}{LongAlpaca-7B-16k} & - & 0 & 0 & 0 & 0 & \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{} & \checkmark & 0 & 0 & 0 & 0 & \xmark	& \xmark	& \xmark \\
%     \midrule
%     \multicolumn{1}{l}{long\_llama\_code\_7b} & - & 0.2 &	3.2 &	3.4 &	2.6 &	2.6 &	2.4 &	1.8  \\
%     \multicolumn{1}{l}{} & \checkmark & 1.6 &	2.2 &	1.6 &	2.8 &	2.2 &	2.0 &	3.0  \\
%     \midrule
%     \multicolumn{1}{l}{chatglm3-6b-32k} & - & 1.6 & 4.6	& 4.4	& 3.2	& 1.0	& 2.4	& 2.4  \\
%     \multicolumn{1}{l}{} & \checkmark & 5.0 & 4.2	& 3.4	& 4.8	& 5.4	& 3.6	& 3.4  \\
%     \midrule
%     \multicolumn{1}{l}{Yi-6B-200K} & - & 0	& 3.0	& 0.6	& \xmark	& \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{} & \checkmark & 0	& 0.2	& 1.6	& \xmark	& \xmark	& \xmark	& \xmark \\
%     \midrule
%     %\multicolumn{1}{l}{Baichuan2-7B-Base} & - & 0	& 3.8	& 0	& 	0	& 	0	& 	0	& 	0 \\
%     %\multicolumn{1}{l}{} & \checkmark & 0	& 2.4	& 0	& 	0	& 	0	& 	0	& 	0 \\
%     %\midrule
%     \multicolumn{1}{l}{internlm2-base-7b} & - & 0	& 0.8	& 0	& 0	& \xmark 	& \xmark	& \xmark\\
%     \multicolumn{1}{l}{} & \checkmark & 3.0	& 0.2	& 0	& 0	& \xmark 	& \xmark	& \xmark\\
%     \midrule
%     \multicolumn{1}{l}{Qwen-7B} & - & 0.2	& 2.4 &	3.0 &	3.6 &	2.4 &	2.6 &	2.6 \\
%     \multicolumn{1}{l}{} & \checkmark & 2.0	& 1.0 &	1.6 &   1.2 &	1.8 &	2.6 &	2.8 \\
%     \midrule
%     \multicolumn{1}{l}{Mistral-7B-v0.1} & - & 0.4	& 0.8	& 3.8	& \xmark	& \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{} & \checkmark & 3.8	& 3.0	& 0.8	& \xmark	& \xmark	& \xmark	& \xmark \\
%     \midrule
%     \multicolumn{1}{l}{gemma-7b} & - & 0 & 2.8 &	3.2 &	0	& \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{} & \checkmark & 0 & 2.0 &	1.4 &	0	& \xmark	& \xmark	& \xmark \\
%     \midrule
%     \multicolumn{1}{l}{rwkv-5-world} & - & 0 & 1.0	& 0.8	& 0	& 0.2	& 0.2	& 0 \\
%     \multicolumn{1}{l}{} & \checkmark & 1.8 & 0.2	& 0.4	& 0	& 0	& 0	& 0 \\
%     \midrule
%     \multicolumn{1}{l}{mamba-2.8b} & - & 0      & 0	& 0	& 0	& 0	& 0	& 0 \\
%     \multicolumn{1}{l}{} & \checkmark & 1.6      & 0	& 0	& 0	& 0	& 0	& 0 \\
%     \midrule
%     \multicolumn{1}{l}{gemini-1.0-pro} & - & 4.0 &	10.8 &	11.2	& 3.4	& 3.8	& 6.0	& 3.6 \\
%     \multicolumn{1}{l}{} & \checkmark & 8.4 & 11.0 &	13.0	& 6.4	& 3.6	& 4.4	& 5.2 \\
%     \midrule
%     \multicolumn{1}{l}{gpt4-turbo} & - & 2.5 &	25.5 &	21.5 &	22.5 &	23.0 &	18.5 &	21.0 \\
%     \multicolumn{1}{l}{} & \checkmark & 21.6 &	21.0 &	17.5 &	16.0 &	12.0 &	9.0 &	14.0 \\
% \bottomrule
% \end{tabular}
% \caption{Ablation study on Discovery dataset to compare the results for including the instruction of label space at the beginning of the prompt. \textbf{Label Instruction} means including the label space in the instructions.}
% \label{table:label_instruction_result}
% \end{table}



==> Sections_old/discovery_results.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{10K}} &\multicolumn{1}{c}{\textbf{20K}}  &\multicolumn{1}{c}{\textbf{30K}}    &\multicolumn{1}{c}{\textbf{40K}}  &\multicolumn{1}{c}{\textbf{50K}}  \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 0  & 0	& 0	& 0	& \xmark	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32k & 0  & 1.0	& 0	& \xmark	& \xmark  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200k & 0  & 0 & 0	& 0	& 0 \\

% \multicolumn{1}{l}{Baichuan2-7B-Base} & 7B & 4k & 0  &  \xmark &  \xmark	&  \xmark	&  \xmark \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 0  & 0	& 0	& 0	& 0  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 0  & 0.2	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\

\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 0  & 0	& 0	& \xmark &  \xmark \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{1.5}  & \textbf{0.5}	& \textbf{0.5}	& \textbf{0.5}	& \textbf{0.5} \\

\midrule

\multicolumn{1}{l}{SoTA (MTL)} & N/A & - & \multicolumn{5}{c}{\textbf{87.4}} \\

\bottomrule
\end{tabular}
\caption{Discovery Result.}
\label{table:discovery_result}
\end{table}




==> Sections_old/exploratory_tacred.tex <==
% \begin{table}[!thb]
%     \small
%     \centering
%     \begin{tabular}{cccccccc}
%     \toprule
%     \multicolumn{1}{l}{\textbf{Model}} 
%     &\multicolumn{1}{c}{\textbf{2k}} &\multicolumn{1}{c}{\textbf{5k}}  &\multicolumn{1}{c}{\textbf{10k}}    &\multicolumn{1}{c}{\textbf{15k}}  &\multicolumn{1}{c}{\textbf{20k}}   &\multicolumn{1}{c}{\textbf{25k}} &\multicolumn{1}{c}{\textbf{32k}}               \\
%     \midrule
%     \multicolumn{1}{l}{LLaMA-2-7B-32K} & 0.4	& 3.7	& 0.7	& 2.2	& 3.8	& 5.7	& 0   \\
%     \multicolumn{1}{l}{w. G} & 0.2 & 5.6 & 1.0  & 1.1 &	3.8 & 3.2 &	0   \\
%     \midrule
%     \multicolumn{1}{l}{LongAlpaca-7B-16k} & 0 & 0 & 0 & 0 & \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{w. G} & 0 & 0 & 0 & 0 & \xmark	& \xmark	& \xmark \\
%     \midrule
%     \multicolumn{1}{l}{long\_llama\_code\_7b} & 1.8	& 5.1	& 4.9	& 5.7	& 4.4	& 5.2	& 4.3  \\
%     \multicolumn{1}{l}{w. G} & 2.0 &	2.5 &	1.3 &	3.4 &	3.1 &	2.8 &	2.4  \\
%     \midrule
%     \multicolumn{1}{l}{chatglm3-6b-32k} & 38.0	& 51.3	& 48.9	& 43.7	& 46.5	& 45.0	& 39.4  \\
%     \multicolumn{1}{l}{w. G} & 33.8 & 45.3	& 44.0	& 41.2	& 44.9	& 36.1	&  35.0 \\
%     \midrule
%     \multicolumn{1}{l}{Yi-6B-200K} & 0	& 3.0	& 0.6	& \xmark	& \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{w. G}       & 0  & 0 & 0	& \xmark	& \xmark	& \xmark	& \xmark \\
%     \midrule
%     %\multicolumn{1}{l}{Baichuan2-7B-Base} & 14.6	& 10.9	& 0	& 0	& 0	& 0	& 0 \\
%     %\multicolumn{1}{l}{w. G}            & 0	& 0.5	& 0	& 	0	& 	0	& 	0	& 	0 \\
%     %\midrule
%     \multicolumn{1}{l}{internlm2-base-7b} & 0 & 0 & 0	& 0	& \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{w. G}              & 0 & 0 & 0	& 0	& \xmark 	& \xmark	& \xmark\\
%     \midrule
%     \multicolumn{1}{l}{Qwen-7B} & 2.6	& 2.7	& 2.9	& 2.3	& 4.5	& 2.4	& 3.0 \\
%     \multicolumn{1}{l}{w. G}    &  2.4	&  0.4  & 1.2   & 0.7   & 1.2   & 1.6   & 1.4 \\
%     \midrule
%     \multicolumn{1}{l}{Mistral-7B-v0.2-base} &  	&       &     &  	&  	& 	&   \\
%     \multicolumn{1}{l}{w. G}                 &   	&   	&     &     & 	& 	&   \\
%     \midrule
%     \multicolumn{1}{l}{gemma-7b} & 0	& 0	& 0	& 0	& \xmark	& \xmark	& \xmark \\
%     \multicolumn{1}{l}{w. G} &  0.1 & 0 &	0 &	0	& \xmark	& \xmark	& \xmark \\
%     \midrule
%     \multicolumn{1}{l}{rwkv-5-world} & 2.0	& 3.1	& 0.4	& 0.4	& 1.8	& 3.1	& 1.8 \\
%     \multicolumn{1}{l}{w. G}         & 1.6 & 4.7	& 3.6	& 4.0	& 4.0   & 4.0	& 3.8 \\
%     \midrule
%     \multicolumn{1}{l}{mamba-2.8b}   & 0      & 0	& 0	& 0	& 0	& 0	& 0 \\
%     \multicolumn{1}{l}{w. G}         & 0 & 0 & 0	& 0 & 0 & 0	& 0 \\
%     \midrule
%     \multicolumn{1}{l}{gemini-1.0-pro} & 62.3	& 71.4	& 77.8	& 78.2	& 76.8	& 75.2	& 73.7 \\
%     \multicolumn{1}{l}{w. G}           & - & - &	-	& -	& -	& -	& - \\
%     \midrule
%     \multicolumn{1}{l}{gpt4-turbo} & 74.4 &	80.1 &	81.3 &	84.2 &	84.3 &	83.9 &	83.0 \\
%     \multicolumn{1}{l}{w. G}           & - & - &	-	& -	& -	& -	& - \\
%     \bottomrule
% \end{tabular}
% \caption{Exploratory study on TacRED dataset to compare the results for position distribution. \textbf{w. G} means grouping the same-type instances to clusters.}
% \label{table:label_instruction_result}
% \end{table}

\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{Scatter}} &\multicolumn{1}{c}{\textbf{Grouped}}  &\multicolumn{1}{c}{\textbf{$\Delta$}}                \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{3}{c}{\textbf{10K}}            \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0  & 0 & 0	 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 0.4  & 3.0	& +2.6 \\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & 38.9  & 35.6  & -3.3 \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 45.2  & 33.0 & -12.2\\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 51.6  & 5.1 & -46.5 \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0 & 0\\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 8.0  & 0 & -8 \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 15.5  & 4.8  & -9.7 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 4.1  & 0  & -4.1 \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 1.0  & 3.6  & +2.6 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0 \\

\midrule

% \multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & -  & -	& - \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K   & 79.5  & 59.2	& -20.3 \\



\bottomrule
\end{tabular}
\caption{Exploratory Result on TacRED 3 Round. \textbf{Grouped} means forcing the same-typed demonstration examples near by each other instead of randomly distributing in the prompt.}
\label{table:label_instruction_result}
\end{table}

==> Sections_old/go_emotion_results.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{0.8K}} &\multicolumn{1}{c}{\textbf{1.6K}}  &\multicolumn{1}{c}{\textbf{2.4K}}    &\multicolumn{1}{c}{\textbf{3.2K}}  &\multicolumn{1}{c}{\textbf{4K}}  \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 0  & 0	& 0	& 0.2	& 0.2	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & \textbf{22.0}  & 17.0	& 15.0	& 12.6	& 10.6  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 14.8  & \textbf{18.2}	& \textbf{18.6}	& \textbf{19.0}	& \textbf{14.2} \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 2.6  & 11.4	& 7.4	& 11.6	& 12.4 \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 0  & 0	& 0.8	& 4.0	& 4.0 \\

% \multicolumn{1}{l}{Baichuan2-7B-Base} & 7B & 4k & 3.2  & 2.8 & 4.4	& 4.2	& 5.2 \\
\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 0  & 0	& 0	& 0.2	& 0.4  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 8.8  & 7.4	& 4.6	& 5.2	& 4.0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\
\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K &  20.3  & 21.4	& 22.4	& 24.4	& 24.0 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{36.5}  & \textbf{34.4}	&  \textbf{35.0}	&  \textbf{33.3}	& \textbf{32.0} \\

\midrule
\multicolumn{1}{l}{SoTA (BERT)} & N/A & - & \multicolumn{5}{c}{\textbf{58.9}} \\

\bottomrule
\end{tabular}
\caption{GoEmotion Result.}
\label{table:goemo_result_new}
\end{table}

==> Sections_old/merged_1.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{2K}} &\multicolumn{1}{c}{\textbf{4K}}  &\multicolumn{1}{c}{\textbf{7K}}    &\multicolumn{1}{c}{\textbf{9K}}  &\multicolumn{1}{c}{\textbf{14K}}  \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & \textbf{30.2}  & \textbf{70.4} & \textbf{72.0}	& \textbf{75.6}	& \textbf{77.2}	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & 16.6  & 23.2	& 22.4	& 22.8	& 8.8  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 21.6  & 52.8	& 61.4	& 66.0	& 67.8 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 29.8  & 43.6	& 66.4	& 67.8	& 64.0 \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 25.8  & 0	& 0	& 0	& 1.2 \\

\multicolumn{1}{l}{Yi-34B-200K} & 6B & 200K & 4.2  & 1.0	& 0.6	& 1.2	& 3.4 \\

% \multicolumn{1}{l}{Baichuan2-7B-Base} & 7B & 4k & 3.2  & 2.8 & 4.4	& 4.2	& 5.2 \\
\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 5.6  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 3.0  & 19.4	& 28.0	& 31.6	& 32.6  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 8.6  & 21.2	& 0.4	& 0	& 0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\


\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 33.4  & 41.4	& 40.6	&  45.6	& 50.2 \\
\multicolumn{1}{l}{Claude3-Opus} & N/A & 200K & 55.0  & 54.8	& 44.0	&  26.4	&  14.0 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{73.5}  & \textbf{80.5}	& \textbf{82.0}	&  \textbf{83.5}	&  \textbf{84.4} \\


\midrule
\multicolumn{1}{l}{SoTA (RoBERTA + ICDA)} & N/A & - & \multicolumn{5}{c}{\textbf{94.4}} \\

\bottomrule
\end{tabular}
\vspace{-1ex}
\caption{BANKING77 result with respect to increasing context length. \textbf{1R} represents one round of traversing all the instances with unique label.}
\label{tab:bank77}
\vspace{1ex}

\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{4K}} &\multicolumn{1}{c}{\textbf{7K}}  &\multicolumn{1}{c}{\textbf{10K}}    &\multicolumn{1}{c}{\textbf{14K}}  &\multicolumn{1}{c}{\textbf{18K}}               \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0.4  & 0.4	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 0  & 0.4	& 0.4	& 0.8	& 0.4	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & 29.7  & 36.1	& 38.9	&  40.1 & 25.2 \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 38.7  &	47.3 & 45.2 & 43.6	& 40.6 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & \textbf{53.3}  & \textbf{53.1}	& \textbf{51.6}	& \textbf{48.0}	& \textbf{42.3} \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 5.6  & 1.9	& 8.0	& 9.5	& 2.0 \\

\multicolumn{1}{l}{Yi-34B-200K} & 34B & 200K & 50.2  & 49.8	& 47.4	& 43.4	& 41.9 \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 29.6  & 27.2	& 15.5	& 10.7	& 8.0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 3.8  & 7.1	& 4.1	& 6.6	& 4.9  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 1K & 2.3  & 2.6	& 1.0	& 0	& 1.2 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\

\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 71.4  & 77.8	& 78.2	& 77.4	& 76.8 \\

\multicolumn{1}{l}{Claude3-Opus} & N/A & 200K & 68.7  & 74.1	& 33.9	& 41.8	& 43.7 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K   & \textbf{74.4}  & \textbf{76.5}	& \textbf{79.5}	& \textbf{80.4}	&  \textbf{84.2} \\

\midrule
\multicolumn{1}{l}{SoTA (DeepStruct)} & N/A & - & \multicolumn{5}{c}{76.8} \\


\bottomrule
\end{tabular}
\vspace{-1ex}
\caption{TacRED result with respect to increasing context length.}
\label{tab:tacred}


\end{table}

==> Sections_old/merged_2.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{8K}} &\multicolumn{1}{c}{\textbf{13K}}  &\multicolumn{1}{c}{\textbf{19K}}    &\multicolumn{1}{c}{\textbf{25K}}  &\multicolumn{1}{c}{\textbf{32K}}               \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 16.3 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 6.9 & 13.9	& 6.3	& 5.7	& 5.9\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & 5.1 & 8.9	& 8.8	& 12.4	& 10.4  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 14.4 & 18.4	& 15.5	& 16.4	& 13.2 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & \textbf{24.3} & \textbf{23.2}	& \textbf{23.4}	& \textbf{22.3}	& \textbf{21.2} \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 0 & 0	& 0.8	& 0.8	& 0 \\

\multicolumn{1}{l}{Yi-34B-200K} & 34B & 200K & 29.2 & 25.9	& 26.6	& 29.7	& 29.4 \\

% \multicolumn{1}{l}{Baichuan2-7B-base} & 7B & 192K & 0 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 12.2 & 13.4 & 6.4 & 2.1 & 1.1 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 4.0 & 3.8	& 3.0	& 6.4	& 2.2 \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 0 & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0 & 0	& 0	& 0	& 0 \\

\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 23.6 & 29.2	& 33.2	& 26.1	& 17.3 \\

\multicolumn{1}{l}{Claude3-Opus} & N/A & 200K & 28.4 & 47.2	& 25.2	& 1.5	& 0 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{43.5} & \textbf{48.8} & \textbf{53.6} & \textbf{60.2} & \textbf{60.9} \\

\midrule

\multicolumn{1}{l}{SoTA (HiDialog)} & N/A & - & \multicolumn{5}{c}{\textbf{77.1}} \\

\bottomrule
\end{tabular}
\vspace{-1ex}
\caption{DialogRE result with respect to increasing context length.}
\label{tab:dial}
\vspace{1ex}


\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{10K}} &\multicolumn{1}{c}{\textbf{20K}}  &\multicolumn{1}{c}{\textbf{30K}}    &\multicolumn{1}{c}{\textbf{40K}}  &\multicolumn{1}{c}{\textbf{50K}}  \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 0  & 0	& 0	& 0	& \xmark	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32k & 0  & 1.0	& 0	& \xmark	& \xmark  \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200k & 0  & 0 & 0	& 0	& 0 \\
\multicolumn{1}{l}{Yi-34B-200K} & 34B & 200K & 0  & -	& 0	& -	& - \\

% \multicolumn{1}{l}{Baichuan2-7B-Base} & 7B & 4k & 0  &  \xmark &  \xmark	&  \xmark	&  \xmark \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 0  & 0	& 0	& 0	& 0  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 4K & 0  & 0.2	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\

\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 0  & 0	& 0	& \xmark &  \xmark \\

\multicolumn{1}{l}{Claude3-Opus} & N/A & 200K & 1.2  & \textbf{0.6}	& \textbf{0.6}	& \textbf{0.6} &  0.2 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K & \textbf{1.5}  & 0.5	& 0.5	& 0.5	& \textbf{0.5} \\

\midrule

\multicolumn{1}{l}{SoTA (MTL)} & N/A & - & \multicolumn{5}{c}{\textbf{87.4}} \\

\bottomrule
\end{tabular}
\vspace{-1ex}
\caption{Discovery result with respect to increasing context length.}
\label{tab:disc}

\end{table}

==> Sections_old/models.tex <==
\begin{table}[!tbh]
\small
\begin{tabular}{llllll}
\toprule
Model                & Size & Initialization & Strategy                 & Train & Support \\
\midrule
\defcitealias{team2024gemma}{Gemma-7B-base}\citetalias{team2024gemma}        
& 7B   & Gemma          &  RoPE + LF    & 8K    & 8K      \\
\defcitealias{Liu2023LostIT}{LLaMA-2-7B-32K}\citetalias{Liu2023LostIT}    
& 7B   & LLaMA-2        & Position Interpolation   & 32K   & 32K     \\
\defcitealias{zeng2022glm}{ChatGLM3-6B-32K}\citetalias{zeng2022glm}
& 6B   & ChatGLM        & Position Encoding Scheme & 32K   & 32K     \\
\defcitealias{bai2023qwen}{Qwen-1.5-7B-base}\citetalias{bai2023qwen}
& 7B   & Qwen           & NTK-Aware Interpolation  & 32K   & 32K     \\
\defcitealias{jiang2023mistral}{Mistral-7B-v0.2-base}\citetalias{jiang2023mistral}
& 7B   & Mistral        & LF                       & 32K   & 32K     \\
\defcitealias{Chen2023LongLoRAEF}{LLaMA-2-7B-LongLora}\citetalias{Chen2023LongLoRAEF}
& 7B   & LLaMA-2        & Shifted Short Attention  & 100K  & 100K     \\
%Baichuan2-7B-base    & 7B   & Baichuan       & -                        & -     & 192K    \\
\defcitealias{ai2024yi}{Yi-6B-200K}\citetalias{ai2024yi}
& 6B   & Yi             & Position Interpolation +LF   & 200K  & 200K    \\
\defcitealias{cai2024intern}{InternLM2-7B-base}\citetalias{cai2024intern}
& 7B   & InternLM       & Dynamic NTK              & 32K   & 200K   \\
\defcitealias{tworkowski2023focused}{Long-LLaMA-code-7B}\citetalias{tworkowski2023focused}
& 7B   & LLaMA-2        & Focused Transformer      & 8K    & 256K    \\
\midrule
\defcitealias{peng2023rwkv}{RWKV-5-World}\citetalias{peng2023rwkv}
& 3B   & RWKV           & Attention-free Model     & 4K    & $\infty$       \\
\defcitealias{gu2023mamba}{Mamba-2.8B}\citetalias{gu2023mamba}
& 2.8B & Mamba          & State Space Model        & 2K    & $\infty$       \\
\midrule
\defcitealias{team2023gemini}{Gemini-1.0-Pro}\citetalias{team2023gemini}
& -    & Gemini         & Ring Attention           & 32K   & 32K     \\
\defcitealias{achiam2023gpt}{GPT4-turbo}\citetalias{achiam2023gpt}
& -    & GPT-4          & -                        & -     & 128K    \\
\bottomrule
\end{tabular}
\caption{The overview of the evaluated models. We utilize base models before instruction-tuning except Gemini and GPT4-turbo. LF means fine-tuning the model on longer-context corpus after pre-training. }
\vspace{-3ex}
\label{tab:models}
\end{table}

==> Sections_old/tacred_results.tex <==
\begin{table}[tbh]
\small
\centering
\begin{tabular}{lccccccc}

\toprule
\multicolumn{1}{l}{\textbf{Model}} &\multicolumn{1}{c}{\textbf{Param}}
&\multicolumn{1}{c}{\textbf{Support}}  &\multicolumn{1}{c}{\textbf{1R}} &\multicolumn{1}{c}{\textbf{2R}}  &\multicolumn{1}{c}{\textbf{3R}}    &\multicolumn{1}{c}{\textbf{4R}}  &\multicolumn{1}{c}{\textbf{5R}}               \\
\midrule
\multicolumn{1}{l}{\textbf{Context Tokens}} &\multicolumn{1}{c}{\textbf{}}
&\multicolumn{1}{c}{\textbf{}}  &\multicolumn{1}{c}{\textbf{4K}} &\multicolumn{1}{c}{\textbf{7K}}  &\multicolumn{1}{c}{\textbf{10K}}    &\multicolumn{1}{c}{\textbf{14K}}  &\multicolumn{1}{c}{\textbf{18K}}               \\
\midrule

\multicolumn{1}{l}{Gemma-7B-base} & 7B & 8K & 0.4  & 0.4	& 0	& 0	& 0 \\

\multicolumn{1}{l}{LLaMA-2-7B-32K} & 7B & 32K & 0  & 0.4	& 0.4	& 0.8	& 0.4	\\

\multicolumn{1}{l}{ChatGLM3-6B-32K} & 6B & 32K & 29.7  & 36.1	& 38.9	&  40.1 & 25.2 \\

\multicolumn{1}{l}{Qwen-1.5-7B-base} & 7B & 32K & 38.7  &	47.3 & 45.2 & 43.6	& 40.6 \\

\multicolumn{1}{l}{Mistral-7B-v0.2-base} & 7B & 32K & \textbf{53.3}  & \textbf{53.1}	& \textbf{51.6}	& \textbf{48.0}	& \textbf{42.3} \\

\multicolumn{1}{l}{LLaMA-2-7B-LongLora} & 7B & 100K & 0  & 0	& 0	& 0	& 0 \\

\multicolumn{1}{l}{Yi-6B-200K} & 6B & 200K & 5.6  & 1.9	& 8.0	& 9.5	& 2.0 \\

\multicolumn{1}{l}{InternLM2-7B-base} & 7B & 200K & 29.6  & 27.2	& 15.5	& 10.7	& 8.0 \\

\multicolumn{1}{l}{Long-LLaMA-code-7B} & 7B & 256K & 3.8  & 7.1	& 4.1	& 6.6	& 4.9  \\

\midrule

\multicolumn{1}{l}{RWKV-5-World} & 7B & 1K & 2.3  & 2.6	& 1.0	& 0	& 1.2 \\

\multicolumn{1}{l}{Mamba-2.8B} & 2.8B & 2K & 0  & 0	& 0	& 0	& 0 \\

\midrule

\multicolumn{1}{l}{Gemini-1.0-Pro} & N/A & 32K & 71.4  & 77.8	& 78.2	& 77.4	& 76.8 \\

\multicolumn{1}{l}{GPT4-turbo} & N/A & 128K   & \textbf{74.4}  & \textbf{80.1}	& \textbf{81.3}	& \textbf{83.2}	&  \textbf{84.3} \\

\midrule
\multicolumn{1}{l}{SoTA (DeepStruct)} & N/A & - & \multicolumn{5}{c}{76.8} \\


\bottomrule
\end{tabular}
\caption{TacRED Result.}
\label{table:tacred_result}
\end{table}
